Piercing the Veil of TVL: DeFi Reappraised

Total value locked (TVL) is widely used to measure the size and popularity of decentralized finance (DeFi). However, TVL can be easily manipulated and inflated through "double counting" activities such as wrapping and leveraging. As existing methodologies addressing double counting are inconsistent and flawed, we propose a new framework, termed "total value redeemable (TVR)", to assess the true underlying value of DeFi. Our formal analysis reveals how DeFi's complex network spreads financial contagion via derivative tokens, increasing TVL's sensitivity to external shocks. To quantify double counting, we construct the DeFi multiplier, which mirrors the money multiplier in traditional finance (TradFi). This measurement reveals substantial double counting in DeFi, finding that the gap between TVL and TVR reached \$139.87 billion during the peak of DeFi activity on December 2, 2021, with a TVL-to-TVR ratio of approximately 2. We conduct sensitivity tests to evaluate the stability of TVL compared to TVR, demonstrating the former's significantly higher level of instability than the latter, especially during market downturns: A 25% decline in the price of Ether (ETH) leads to a \$1 billion greater non-linear decrease in TVL compared to TVR via the liquidations triggered by derivative tokens. We also document that the DeFi money multiplier is positively correlated with crypto market indicators and negatively correlated with macroeconomic indicators. Overall, our findings suggest that TVR is more reliable and stable than TVL.

==> Algorithms/risk_algo.tex <==
\begin{algorithmic}[1]
    \State Extract ETH and its derivative token list $M$ from $D$
    \ForAll{protocol $i$ in protocol list $I_t$}
        \State Extract token-amount $(c_{n,i,t}, a_{n,i,t})$ pairs for protocol $i$ from $D$
        \ForAll{token-amount pair $(c_{n,i,t}, a_{n,i,t})$}
        % \Comment{TVL and TVR decline due to token price change}
            \If{$c$ is a plain token}
                \State $\Delta TVL \leftarrow \Delta TVL - a_n \cdot d$
                \State $\Delta TVR \leftarrow \Delta TVL - a_n \cdot d$
            \Else
                \State Calculate the weight $\beta$ in the composition of $c$
                \State $\Delta TVL \leftarrow \Delta TVL - a_n \cdot d \cdot \beta$
            \EndIf
            \State Update the token dollar amount $a_{t,n}$ after price change
        \EndFor
        
        \If{the protocol is a PLF}
        % \Comment{TVL and TVR decline due to liquidations}
            \State Extract every account in the PLF $i$ from $D$
            \ForAll{account $a \in \mathcal{A}$}
                \If{Health factor is below the CF-HF threshold}
                    \State $\Delta TVL \leftarrow \Delta TVL - a_n \cdot d \cdot \beta$
                \EndIf
            \EndFor
    
            \If{the protocol is a CDP}
                \If{Total debt value is greater than total collateral value}
                    \State Update crypto-backed stablecoin price after depegging
                \EndIf
            \EndIf

            \ForAll{token-amount pair $(c_{n,i,t}, a_{n,i,t})$}
            % \Comment{TVL and TVR decline due to depegging}
                \If{$c$ is a depeggd crypto-back stablecoins}
                    \State $\Delta TVL \leftarrow \Delta TVL - a_n \cdot \frac{\textnormal{CDP total collateral}}{\textnormal{CDP total debt}}$
                \EndIf
            \EndFor
        \EndIf
    \EndFor
        
\end{algorithmic}


==> Algorithms/tvr_algo.tex <==
\begin{algorithmic}[1]
{
    \State Initialize hash table $H$
    \For{every plain token $f \in \mathcal{F}$}
        \State Insert $f$ into the $H$
    \EndFor
    \State Extract token-amount $(c_n, a_n)$ pairs for all protocols $\mathcal{C}$ from $D$
    \For{$(c_n, a_n) \in \mathcal{C}$}
        \If{$c_n$ in $H$}
            \State $TVR \leftarrow TVR + a_n$
        \EndIf
    \EndFor
}
\end{algorithmic}

==> Equations/collat_constraint.tex <==
\begin{equation}
    \label{eq:collat_constraint}
    p_{c,t}q_{c,t} \geq \alpha L_{t}
\end{equation}

==> Equations/dai_adai.tex <==
\begin{equation}
    \label{eq:dai_adai}
    \begin{split}
        p_{\text{\scriptsize{aDAI}},t}
        = p_{\text{\scriptsize{DAI}},t}
        = \begin{cases} 
          1 & \sum_{v \in \mathcal{V}} p_{v,t}q_{v,t} \geq \sum_{v \in \mathcal{V}} L_{v,t} \\
          \frac{\sum_{v \in \mathcal{V}} p_{v,t}q_{v,t}}{\sum_{v \in \mathcal{V}} L_{v,t}} & \sum_{v \in \mathcal{V}} p_{v,t}q_{v,t} < \sum_{v \in \mathcal{V}} L_{v,t}
        \end{cases} 
    \end{split}
\end{equation}

==> Equations/endo_price_cbs.tex <==
\begin{equation}
    \label{eq:endo_price_cbs} 
    \footnotesize
    \begin{split}
        p_{d,t}(p_{1,t}, p_{2,t},\ldots, p_{\bar{u},t}) &= \begin{cases} 
          \rho_{d,t} + \epsilon_{d,t} & \Gamma_{t} \geq 1 \\
          &\\
          \frac{\displaystyle\sum_{a}\sum_{u} p_{u,t}q_{u,t}}{\displaystyle\sum_{a} q_{d,t}} + \epsilon_{s,t} & \Gamma_{t} < 1 \\
        \end{cases} \\
        &\\
        \Gamma_{t} &= \frac{\displaystyle\sum_{a}\sum_{u} p_{u,t}q_{u,t}}{\displaystyle\sum_{a}\rho_{d,t}q_{d,t}}
    \end{split}
\end{equation}

==> Equations/endo_price_linear.tex <==
\begin{equation}
    \label{eq:endo_price_linear}
    p_{d,t}(p_{1,t}, p_{2,t},\hdots, p_{\bar{u},t}) = \sum_{u} \beta_{u,t} \cdot p_{u,t} + \epsilon_{d,t}
\end{equation}

==> Equations/endo_quantity_derivative.tex <==
\begin{equation}
    \label{eq:endo_quantity_derivative}
    \fontsize{8}{9}\selectfont
    \begin{split}
        &q_{d,t}(p_{1,t}, p_{2,t},\hdots, p_{\bar{u},t}) = \\
        &\sum_{a \in \mathcal{A}}        
        \begin{cases} 
            q_{d,t} & \begin{split}
                h_{d,t}(p_{1,t}, p_{2,t},\hdots, p_{\bar{u},t}) \geq 1 \quad \text{or}\\
                H_{d,t}(p_{1,t}, p_{2,t},\hdots, p_{\bar{u},t}) < 1  
            \end{split}\\
            q_{d,t} (1 - \delta_0) & \psi_{1} \leq h_{d,t}(p_{1,t}, p_{2,t},\hdots, p_{\bar{u},t}) < 1 \\
            q_{d,t} (1 - \delta_1) & \psi_{2} \leq h_{d,t}(p_{1,t}, p_{2,t},\hdots, p_{\bar{u},t}) < \psi_{1} \\
            & \vdots \\
            q_{d,t} (1 - \delta_{n-1}) & \psi_{n} \leq h_{d,t}(p_{1,t}, p_{2,t},\hdots, p_{\bar{u},t}) < \psi_{n - 1}\\
            q_{d,t} (1 - \delta_{n}) & \begin{split}
                h_{d,t}(p_{1,t}, p_{2,t},\hdots, p_{\bar{u},t}) < \psi_{n} \quad \text{and}\\
                H_{d,t}(p_{1,t}, p_{2,t},\hdots, p_{\bar{u},t}) \geq 1
            \end{split}\\
        \end{cases}\\
        &h_{d,t}(p_{1,t}, p_{2,t},\hdots, p_{\bar{u},t}) = \frac{\displaystyle\sum_{d \in \mathcal{F}^{\complement}_{t}\cap\mathcal{T}_{a}}\alpha p_{d,t}(p_{1,t}, p_{2,t},\hdots, p_{\bar{u},t})q_{d,t}}{\displaystyle\sum_{b \in \mathcal{D}_{a}} p_{b,t}(p_{1,t}, p_{2,t},\hdots, p_{\bar{u},t})q_{b,t}}\\
        &H_{d,t}(p_{1,t}, p_{2,t},\hdots, p_{\bar{u},t}) = \frac{\displaystyle\sum_{d \in \mathcal{F}^{\complement}_{t}\cap\mathcal{T}_{a}}p_{d,t}(p_{1,t}, p_{2,t},\hdots, p_{\bar{u},t})q_{d,t}}{\displaystyle\sum_{b \in \mathcal{D}_{a}} p_{b,t}(p_{1,t}, p_{2,t},\hdots, p_{\bar{u},t})q_{b,t}}
    \end{split}
\end{equation}


==> Equations/events.tex <==
\begin{equation}
    \label{eq:events}
    
\end{equation}

==> Equations/ind_tvl.tex <==
\begin{equation}
    {\it TVR}_{i} = \underbrace{\sum_{j \in \mathcal{A}_{i}} R_{j}}_{\textnormal{Total Receivables}} \underbrace{- \qquad \sum_{j \in \mathcal{A}_{i}} P_{j}}_{\textnormal{Total Payables}}
    \label{eq:ind_tvr}
\end{equation}

==> Equations/lido_slashing.tex <==
\begin{equation}
    \label{eq:lido_slashing}
    \Delta q_{\text{Lido},\text{ETH}}(S,T) = - \mathcal{P}_{\text{init}} - \mathcal{P}_{\text{corr}}(S,T) -\mathcal{P}_{\text{off}}(T).
\end{equation}

==> Equations/liquidation.tex <==
\begin{equation}
    \label{eq:liquidation}
    l_{t} = \frac{\alpha L_{t} - p_{c,t}q_{c,t}}{\alpha - 1}
\end{equation}

==> Equations/liquidation_events.tex <==
\begin{equation}
    \label{eq:liquidation_event}
    \begin{split}
        &\mathcal{A}_{v,t} = \{q_{v,t} \geq a(L_{v,t})\}\\
        &\mathcal{B}_{v,t} = \{b(L_{v,t}) \leq q_{v,t} \leq a(L_{v,t})\}
    \end{split}
\end{equation}

==> Equations/multiplier.tex <==
\begin{equation}
    M^{DeFi} = \frac{TVL}{TVR}
    \label{eq:multiplier}
\end{equation}

==> Equations/nested_func.tex <==
\begin{equation}
    \label{eq:nested_func}
    \tiny
    p_{d}(p_{1}, p_{2},\ldots, p_{i}) = \left[p_{d} \circ p_{d_1} \ldots \circ p_{d_j}\right](p_{1}, p_{2},\ldots, p_{i}),
\end{equation}

==> Equations/snowballing_tvl.tex <==
\begin{equation}
\scriptsize
\begin{split}
    \label{eq:snowballing_tvl}
    \Delta_{TVL}(d_{\text{ETH}}) &= \underbrace{q^\text{L} p (1-d_{\text{ETH}})}_{\text{\normalfont Lido Pool Value Decline}} + \underbrace{\sum_{c \in C^\text{M}}\sum_v q^\text{M}}_{\text{\normalfont MakerDAO Vaults TVL}}- \underbrace{\sum_{c \in C^\text{M}}\sum_{v \in \mathcal{A}} q^\text{M} p (1-d_{\text{ETH}})}_{\text{\normalfont{Safe Vaults Value}}}\\ 
    &- \underbrace{\sum_{c \in C^\text{M}}\sum_{v \in \mathcal{B}} p (1-d_{\text{ETH}}) (q^\text{M} - \frac{(\alpha L - p (1-d_{\text{ETH}}) q^\text{M})}{p (1-d_{\text{ETH}})(\alpha - 1)})}_{\text{\normalfont{Risky Vaults Value after Liquidation}}}
\end{split}
\end{equation}

==> Equations/snowballing_tvr.tex <==
\begin{equation}
    \scriptsize
    \label{eq:snowballing_tvr}
    \begin{split}
        \Delta_{TVR}(d_{\text{ETH}}) &= \underbrace{q^\text{L} p (1-d_{\text{ETH}})}_{\text{\normalfont Lido Pool Value Decline}} + \underbrace{\sum_{c \in C^\text{M} \cap F}\sum_v q^\text{M}}_{\text{\normalfont MakerDAO Vaults TVR}}- \underbrace{\sum_{c \in C^\text{M} \cap F}\sum_{v \in \mathcal{A}} q^\text{M} p (1-d_{\text{ETH}})}_{\text{\normalfont{Safe Non-derivative Vaults Value}}}\\ 
        &- \underbrace{\sum_{c \in C^\text{M} \cap F}\sum_{v \in \mathcal{B}} p (1-d_{\text{ETH}}) (q^\text{M} - \frac{(\alpha L - p (1-d_{\text{ETH}}) q^\text{M})}{p (1-d_{\text{ETH}})(\alpha - 1)})}_{\text{\normalfont{Risky Non-derivative Vaults Value after Liquidation}}}
    \end{split}
\end{equation}

==> Equations/system_tvl.tex <==
\begin{equation}
    \tiny
    \label{eq:system_tvl}
            {\it TVL}(p_{1}, \hdots, p_{k}) = \sum_{i \in \overline{\mathcal{P}}}
            \left[
                \sum_{j \in \mathcal{F} \cap \mathcal{T}_{i}}p_{j}\cdot q_{j} 
                + \sum_{j \in \overline{\mathcal{F}}\cap \mathcal{T}_{i}}p_{j}(p_{1}, \hdots, p_{n})\cdot q_{j}
            \right] + \sum_{i \in \mathcal{P}}
            \left[
                \sum_{j \in \overline{\mathcal{F}}\cap \mathcal{T}_{i}}p_{j}\cdot q_{j}(p_{j})+\sum_{j \in \overline{\mathcal{F}}\cap \mathcal{T}_{i}}p_{j}(p_{1}, \hdots, p_{n})\cdot q_{j}(p_{1}, \hdots, p_{n})
            \right],
\end{equation}

==> Equations/threshold.tex <==
\begin{equation}
    \label{eq:threshold_liq}
    a(L_t) = \frac{\alpha L_{t}}{q_{c,t}} \quad b(L_t) = \frac{L_{t}}{q_{c,t}}
\end{equation}

==> Exhibits/ana_pip.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{Figures/data_pip.pdf}
    \caption{Data pipeline setup overview.}
    \label{fig:ana_pip}
\end{figure}

==> Exhibits/bal.tex <==
\begin{table}[h]
    \tiny
    \caption{Balance sheets of sample protocols}
    \centering
        \begin{subtable}[h]{0.8\linewidth}
            \input{Tables/bal_AaveV2}
            \subcaption{Balance sheet of Aave}
        \end{subtable}

        \begin{subtable}[h]{0.8\linewidth}
            \input{Tables/bal_Balancer}
            \subcaption{Balance sheet of Balancer}
        \end{subtable}

        \begin{subtable}[h]{0.8\linewidth}
            \input{Tables/bal_CompoundV2}
            \subcaption{Balance sheet of Compound}
        \end{subtable}

        \begin{subtable}[h]{0.8\linewidth}
            \input{Tables/bal_CurveV1}
            \subcaption{Balance sheet of Curve}
        \end{subtable}

        \begin{subtable}[h]{0.8\linewidth}
            \input{Tables/bal_MakerDAO}
            \subcaption{Balance sheet of MakerDAO}
        \end{subtable}

        \begin{subtable}[h]{0.8\linewidth}
            \input{Tables/bal_Yearn}
            \subcaption{Balance sheet of Yearn}
        \end{subtable}
        
    \label{tab:my_label}
\end{table}

==> Exhibits/bal_aave.tex <==
\begin{table}[h]
    \centering
    \input{Tables/bal_AaveV2}
    \caption{Balance sheet of Aave}
    \label{tab:bal_aave}
\end{table}

==> Exhibits/bal_balancer.tex <==
\begin{table}[h]
    \centering
    \input{Tables/bal_Balancer}
    \caption{Balance sheet of Balancer}
    \label{tab:bal_balancer}
\end{table}

==> Exhibits/bal_compound.tex <==
\begin{table}[h]
    \centering
    \input{Tables/bal_CompoundV2}
    \caption{Balance sheet of Compound}
    \label{tab:bal_compound}
\end{table}

==> Exhibits/bal_curve.tex <==
\begin{table}[h]
    \centering
    \input{Tables/bal_CurveV1}
    \caption{Balance sheet of Curve}
    \label{tab:bal_curve}
\end{table}

==> Exhibits/bal_makerdao.tex <==
\begin{table}[h]
    \centering
    \input{Tables/bal_MakerDAO}
    \caption{Balance sheet of MakerDAO}
    \label{tab:bal_makerdao}
\end{table}

==> Exhibits/bal_yearn.tex <==
\begin{table}[h]
    \centering
    \input{Tables/bal_Yearn}
    \caption{Balance sheet of Yearn}
    \label{tab:bal_yearn}
\end{table}

==> Exhibits/bookkeeping.tex <==
\begin{figure*}[tbp]
  \centering
  \begin{minipage}[t]{0.25\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/t-borrow-makerdao.pdf}
    \caption{Borrow.}
    \label{subfig:t-borrow-makerdao}
  \end{minipage}%
  \hfill
  \begin{minipage}[t]{0.25\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/t-borrow-aave.pdf}
    \caption{Borrow.}
    \label{subfig:t-borrow-aave}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.25\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/t-deposit.pdf}
    \caption{Deposit.}
    \label{subfig:t-deposit}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/t-lp.pdf}
    \caption{Provide liquidity.}
    \label{subfig:t-lp}
  \end{minipage}
  \caption{T-accounts of DeFi protocols when users borrow tokens, lend tokens, and issue LP tokens.}
  \label{fig:bookkeeping}
\end{figure*}

==> Exhibits/complexity.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{Figures/complexity.pdf}
    \caption{An example of actions a DeFi user can take to maximize interest, enabled by the \ac{defi} composability.}
    \label{fig:complexity}
\end{figure}

==> Exhibits/defillama-double-count.tex <==
\begin{figure}[H]
      \centering
      \includegraphics[width=\linewidth]{Figures/double-count-removal-20250202.png}
      \caption{DeFiLlama's \ac{tvl} dashboard after deactivating the \enquote{Include in \ac{tvl}: Double Count} toggle. When a user deactivates this toggle, protocols that deposit into another protocol will be excluded from the total \ac{tvl} calculation, and their \ac{tvl} numbers will be displayed in grey.}
      \label{fig:double-count-removal}
\end{figure}

==> Exhibits/defillama_tvl_token_decompose.tex <==
\begin{figure}[tb]
\centering
    \begin{subfigure}{0.8\linewidth}
      \centering
      \includegraphics[width=0.8\linewidth]{Figures/defillama_tvl_token_decompose_makerdao.pdf}
      \caption{MakerDAO.}
      \label{subfig:defillama_tvl_token_decompose_makerdao}
    \end{subfigure}%
    
    \begin{subfigure}{0.8\linewidth}
      \centering
      \includegraphics[width=0.8\linewidth]{Figures/defillama_tvl_token_decompose_aave-v3.pdf}
      \caption{Aave V3.}
      \label{subfig:defillama_tvl_token_decompose_aave-v3}
    \end{subfigure}%
    
    \begin{subfigure}{0.8\linewidth}
      \centering
      \includegraphics[width=0.8\linewidth]{Figures/defillama_tvl_token_decompose_uniswap-v3.pdf}
      \caption{Uniswap V3.}
      \label{subfig:defillama_tvl_token_decompose_uniswap-v3}
    \end{subfigure}
    
      \caption{Token breakdowns of top \ac{cdp}, top lending protocol, and \ac{amm} with the highest \ac{tvl} over time, where the top five tokens contributing the most to the \ac{tvl} are highlighted, while other tokens are grouped under "Others".}
\end{figure}


==> Exhibits/endo_price_example.tex <==
\begin{table}[tb]
\caption{Derivative token price as a function of its underlying tokens in the example system.}
\label{tab:endo_price_example}

\centering
\scriptsize

\input{Tables/endo_price_example}

\end{table}

==> Exhibits/endo_quantity_example.tex <==
\begin{table}[tb]
\caption{Quantity of token staked in the lending protocol or \ac{cdp} as a function of its price in the example system.}
\label{tab:endo_quantity_example}

\centering
\scriptsize

\input{Tables/endo_quantity_example}

\end{table}

==> Exhibits/gov_token_lst.tex <==
\begin{table}[tb] 
  \caption{Governance tokens in Ethereum}
    \begin{center}
    \begin{multicols*}{2} % 开始两栏环境
          \input{Tables/governance_tokens_list}
    \end{multicols*}
    \end{center}
    \label{tab:governance_tokens_list}
\end{table}

==> Exhibits/notation_classification.tex <==
\begin{table}[tb]
    \centering
    \caption{\ac{defi} token classification notations}    
    \label{tab:notation_classification}
    \input{Tables/notation_classification}
\end{table}

==> Exhibits/notation_endo_price.tex <==
\begin{table}[tb]
    \centering
    \caption{Endogenous derivative token price formalization notations}  
    \label{tab:notations_endo_price}
    \input{Tables/notation_endo_price}
\end{table}

==> Exhibits/notation_endo_quantity.tex <==
\begin{table}[tb]
    \centering
    \caption{Endogenous token quantity in \ac{plf} formalization notations}  
    \label{tab:notations_endo_quantity}
    \input{Tables/notation_endo_quantity}
\end{table}

==> Exhibits/notation_formalization.tex <==
\begin{table}[tb]
    \centering
    \caption{\ac{tvl} formalization notations}    
    \label{tab:notation_formalization}
    \input{Tables/notation_formalization}
\end{table}

==> Exhibits/notations.tex <==
\begin{table}[tb]
\footnotesize
\centering
\caption{Mathematical notations in formalization.}
\label{tab:notations}
\input{Tables/notations}

\end{table}

==> Exhibits/on_chain_data.tex <==
\begin{table}[H]
    \centering
    \tiny
    \caption{Statistics of accounts in MakerDAO and Aave on three representative dates.}
    \input{Tables/on_chain_data}
    \label{tab:on_chain_data}
\end{table}

==> Exhibits/params.tex <==
\begin{table}[tb]
    \centering
    \small
    \caption{Default value of parameters.}
    \input{Tables/params}
    \label{tab:params}
\end{table}

==> Exhibits/pie-protocol.tex <==
\begin{figure*}[tbp]
  \centering
  
  \begin{minipage}[t]{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/pie_chart_AAVE_V2.pdf}
    \subcaption{Aave V2.}
    \label{subfig:pie_chart_AAVE_V2}
  \end{minipage}%
  \hfill
  \begin{minipage}[t]{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/pie_chart_BALANCER.pdf}
    \subcaption{Balancer.}
    \label{subfig:pie_chart_BALANCER}
  \end{minipage}%
  \hfill
  \begin{minipage}[t]{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/pie_chart_COMPOUND_V2.pdf}
    \subcaption{Compound V2.}
    \label{subfig:pie_chart_COMPOUND_V2}
  \end{minipage}

  % \vspace{\baselineskip}
  
  \begin{minipage}[t]{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/pie_chart_CURVE.pdf}
    \subcaption{Curve.}
    \label{subfig:pie_chart_CURVE}
  \end{minipage}%
  \hfill
  \begin{minipage}[t]{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/pie_chart_MAKER.pdf}
    \subcaption{MakerDAO.}
    \label{subfig:pie_chart_MAKER}
  \end{minipage}%
  \hfill
  \begin{minipage}[t]{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/pie_chart_Uniswap_V2.pdf}
    \subcaption{Uniswap V2.}
    \label{subfig:pie_chart_Uniswap_V2}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/pie_chart_YEARN.pdf}
    \subcaption{Yearn.}
    \label{subfig:pie_chart_YEARN}
  \end{minipage}
  \caption{Pie charts of token locked in a \ac{defi} protocol.}
  \label{fig:token_locking}
\end{figure*}

==> Exhibits/protocol_specific_tvl.tex <==
\begin{table}[tb]
\caption{Governance token and liquidity pool elements of protocol-specific \ac{tvl} formula for representative protocols.}
\label{tab:protocol_specific_tvl}

\centering
\tiny

\input{Tables/protocol_specific_tvl}

\end{table}

==> Exhibits/risk-analysis.tex <==
\begin{figure}[tp]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/risk_analysis.pdf}
    \caption{All possible pathways for locking ETH into MakerDAO and Lido. The notation "token A-pool/vault-token B" represents users locking token A into the pool or vault to generate token B.}
    \label{fig:risk-analysis}
\end{figure}

==> Exhibits/risk_algo.tex <==
\begin{algorithm}[tb]
\caption{Comparative sensitivity tests for the change in \ac{tvl} and \ac{tvr} in terms of the \ac{eth} price decline}\label{alg:risk_algo}
\footnotesize
\begin{flushleft}
    \textbf{Input:} Protocol list $I_t$, ETH price decline in percentage $d$, and on-chain data $D$;\\
    \textbf{Output:} $\Delta TVL$, $\Delta TVR$;\\
\end{flushleft}

\input{Algorithms/risk_algo}

\end{algorithm}

==> Exhibits/risk_diagram.tex <==
\begin{figure}[tb]
\centering
\includegraphics[width=\linewidth]{Figures/risk_price_decline.pdf}
\caption{$\Delta_{\textit{TVL}}$ and $\Delta_{\textit{TVR}}$ during the \ac{eth} price decline or Lido slashing.}
\label{fig:risk-diagram}
\end{figure}

==> Exhibits/sankey_network.tex <==
\begin{figure}[H]
    \begin{minipage}[tb]{0.49\linewidth}
        \centering
            \begin{subfigure}{\linewidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/tvl_decompose_sankey_max_tvl.pdf}
                \caption{Max \ac{tvl}.}
                \label{subfig:tvl_decompose_sankey_max_tvl}
            \end{subfigure}%
            
            \begin{subfigure}{\linewidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/tvl_decompose_sankey_luna_collapse.pdf}
                \caption{Luna Collapse.}
                \label{subfig:tvl_decompose_sankey_luna_collapse}
            \end{subfigure}
        
            \begin{subfigure}{\linewidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/tvl_decompose_sankey_ftx_collapse.pdf}
                \caption{FTX collapse.}
                \label{subfig:tvl_decompose_sankey_ftx_collapse}
            \end{subfigure}
            
            \caption{Decomposition of \ac{tvl} of the entire \ac{defi} system. We identify four protocols with the highest \ac{tvl} and group the remaining protocols under the category of \enquote{Others}. The band width represents the dollar value of tokens. The blue band represents the \ac{tvl} value, while the orange band represents the \ac{tvr} value.}
        \label{fig:tvl_decompose_sankey}
    \end{minipage}
    \hfill
    \begin{minipage}[tb]{0.49\linewidth}
        \centering
            \begin{subfigure}{0.94\linewidth}
              \centering
              \includegraphics[width=\linewidth]{Figures/network_max_tvl.pdf}
              \caption{Max \ac{tvl}.}
              \label{subfig:network_max_tvl}
            \end{subfigure}%
            
            \begin{subfigure}{0.94\linewidth}
              \centering
              \includegraphics[width=\linewidth]{Figures/network_luna_collapse.pdf}
              \caption{Luna Collapse.}
              \label{subfig:network_luna_collapse}
            \end{subfigure}%
            
            \begin{subfigure}{0.94\linewidth}
              \centering
              \includegraphics[width=\linewidth]{Figures/network_ftx_collapse.pdf}
              \caption{FTX Collapse.}
              \label{subfig:network_ftx_collapse}
            \end{subfigure}
        
        \caption{Token wrapping network of six representative protocols. Node size corresponds to the \ac{tvl}, edge width represents the dollar amount of tokens generated from the source protocol and staked in the target protocol, and node color reflects the ratio between \ac{tvl} and \ac{tvr}. A darker color indicates a higher level of double counting.}
        \label{fig:protocol_network}  
    \end{minipage}
\end{figure}



==> Exhibits/slashing_penalty.tex <==
\begin{table*}[tb]
    \centering
    \scriptsize
    \input{Tables/slashing_penalty}
    \caption{Composition of slashing penalty at different times according to~\cite{Edgington2023UpgradingSlashing}, as denoted by $q_{\text{Lido},\text{ETH}} = - \mathcal{P}_{\text{init}} - \mathcal{P}_{\text{corr}} -\mathcal{P}_{\text{off}}$. $S$ denotes the number of slashed validators. $T$ denotes the total number of active validators. To maintain clarity, we present the constants numerically and do not simplify the equations further.}
    \label{tab:shasling_panalty}
\end{table*} 

==> Exhibits/slashing_test.tex <==
\begin{figure}[H]
\centering
\includegraphics[width=0.9\linewidth]{Figures/sensitivity_slashing_1.pdf}
\caption{Change in \ac{tvl} $\Delta TVL$ and \ac{tvr} $\Delta TVR$ as a function of slashed validators of the biggest node operator in percentage on three representative points.}
\label{fig:sensitivity_test_slashing}
\end{figure}

==> Exhibits/stablecoin_lst.tex <==
\begin{table}[tb] 
  \caption{Algorithmic and fiat-backed stablecoins in Ethereum}
    \begin{center}
    \begin{multicols*}{2} % 开始两栏环境
          \input{Tables/stablecoins_list}
    \end{multicols*}
    \end{center}
    \label{tab:stablecoins_list}
\end{table}

==> Exhibits/sum_stats.tex <==
\begin{table}[tb]
    \centering
    \caption{Summary statistics for the variables computed from the token breakdown data fetched from DeFiLlama. $TVL_{i,t}$ denotes the raw \ac{tvl} for protocol $i$ at time $t$, $TVL^{Adj}_{t}$ denotes the DeFiLlama-adjusted \ac{tvl} for the \ac{defi} system at time $t$, $TVL_t$ denotes the raw \ac{tvl} for the \ac{defi} system, and $TVR_{t}$ denotes the \ac{tvr} at time $t$.}
    \input{Tables/sum_stats}
    \label{tab:sum_stats}
\end{table}

==> Exhibits/tvl-decompo.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/tvl_decomposition.pdf}
    \caption{Decomposition of TVL of the DeFi system of seven mainstream protocols.}
    \label{fig:tvl-decompo}
\end{figure}

==> Exhibits/tvl_subcategory.tex <==
\begin{figure*}[htp]
    \centering
    \begin{subfigure}{0.26\textwidth} 
    \includegraphics[height=0.12\textheight]{Figures/tvl_Ethereum.pdf}
    \caption{Ethereum.}
        \label{fig:tvl_Ethereum}
    \end{subfigure}
    \begin{subfigure}{0.26\textwidth}  
    \includegraphics[height=0.12\textheight]{Figures/tvl_Tron.pdf}
    \caption{Tron.}
        \label{fig:tvl_Tron}
    \end{subfigure}
    \begin{subfigure}{0.26\textwidth}  
    \includegraphics[height=0.12\textheight]{Figures/tvl_Binance.pdf}
    \caption{Binance.}
        \label{fig:tvl_Binance}
    \end{subfigure}
    \begin{subfigure}{0.26\textwidth}     
    \includegraphics[height=0.12\textheight]{Figures/tvl_Arbitrum.pdf}
    \caption{Arbitrum.}  
        \label{fig:tvl_Arbitrum}
    \end{subfigure}
    \begin{subfigure}{0.26\textwidth}    
    \includegraphics[height=0.12\textheight]{Figures/tvl_Polygon}
    \caption{Polygon.}
        \label{fig:tvl_Polygon}
    \end{subfigure}
    \begin{subfigure}{0.26\textwidth}    
    \includegraphics[height=0.12\textheight]{Figures/tvl_Optimism.pdf}
    \caption{Optimism.}
        \label{fig:tvl_Optimism}
    \end{subfigure}
    \begin{subfigure}{0.26\textwidth}    
    \includegraphics[height=0.12\textheight]{Figures/tvl_Avalanche.pdf}
    \caption{Avalanche.}
        \label{fig:tvl_Avalanche}
    \end{subfigure}
    \begin{subfigure}{0.26\textwidth}    
    \includegraphics[height=0.12\textheight]{Figures/tvl_Mixin.pdf}
    \caption{Mixin.}
        \label{fig:tvl_Mixin}
    \end{subfigure}
    \begin{subfigure}{0.26\textwidth}    
    \includegraphics[height=0.12\textheight]{Figures/tvl_Solana.pdf}
    \caption{Solana.}
        \label{fig:tvl_Solana}
    \end{subfigure}
    \caption{DeFiLlama \ac{tvl} with double counting, DeFiLlama \ac{tvl} without double counting, and \ac{tvr} of top nine chains in terms of the DeFiLlama \ac{tvl} without double counting}
    \label{fig:tvl_subcategory}
\end{figure*}

==> Exhibits/tvr_algo.tex <==
\begin{algorithm}[tb]
\caption{\ac{tvr} Measurement Framework}\label{alg:tvr_algo}

\begin{flushleft}
    \textbf{Input:} Set of plain tokens $\mathcal{F}$ and on-chain data $D$;\\
    \textbf{Output:} $TVR$;\\
\end{flushleft}

\input{Algorithms/tvr_algo}

\end{algorithm}

==> Exhibits/tvr_stack_subcategory.tex <==
\begin{figure*}[htp]
    \centering
    \begin{subfigure}{0.26\textwidth} 
    \includegraphics[height=0.12\textheight]{Figures/tvr_stack_Ethereum.pdf}
    \caption{Ethereum.}
        \label{fig:tvr_stack_Ethereum}
    \end{subfigure}
    \begin{subfigure}{0.26\textwidth}  
    \includegraphics[height=0.12\textheight]{Figures/tvr_stack_Tron.pdf}
    \caption{Tron.}
        \label{fig:tvr_stack_Tron}
    \end{subfigure}
    \begin{subfigure}{0.26\textwidth}  
    \includegraphics[height=0.12\textheight]{Figures/tvr_stack_Binance.pdf}
    \caption{Binance.}
        \label{fig:tvr_stack_Binance}
    \end{subfigure}
    \begin{subfigure}{0.26\textwidth}     
    \includegraphics[height=0.12\textheight]{Figures/tvr_stack_Arbitrum.pdf}
    \caption{Arbitrum.}  
        \label{fig:tvr_stack_Arbitrum}
    \end{subfigure}
    \begin{subfigure}{0.26\textwidth}    
    \includegraphics[height=0.12\textheight]{Figures/tvr_stack_Polygon}
    \caption{Polygon.}
        \label{fig:tvr_stack_Polygon}
    \end{subfigure}
    \begin{subfigure}{0.26\textwidth}    
    \includegraphics[height=0.12\textheight]{Figures/tvr_stack_Optimism.pdf}
    \caption{Optimism.}
        \label{fig:tvr_stack_Optimism}
    \end{subfigure}
    \begin{subfigure}{0.26\textwidth}    
    \includegraphics[height=0.12\textheight]{Figures/tvr_stack_Avalanche.pdf}
    \caption{Avalanche.}
        \label{fig:tvr_stack_Avalanche}
    \end{subfigure}
    \begin{subfigure}{0.26\textwidth}    
    \includegraphics[height=0.12\textheight]{Figures/tvr_stack_Mixin.pdf}
    \caption{Mixin.}
        \label{fig:tvr_stack_Mixin}
    \end{subfigure}
    \begin{subfigure}{0.26\textwidth}    
    \includegraphics[height=0.12\textheight]{Figures/tvr_stack_Solana.pdf}
    \caption{Solana.}
        \label{fig:tvr_stack_Solana}
    \end{subfigure}
    \caption{Decomposition of 
    \ac{tvr} of different chains over time}
    \label{fig:tvl_subcategory}
\end{figure*}

==> Exhibits/tvr_total_stack.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/tvr_stack_Total.pdf}
    \caption{Non-derivative tokens locked in the DeFi before 1st June 2023. The rise of governance tokens and NCB stablecoins weakens the dominance of native tokens before October 2020. Three types of tokens remain stable after July 2022 with native tokens and \ac{ncb} tokens almost equally distributed. Three vertical lines mark significant events: the peak TVL on December 2, 2021; the collapse of LUNA on May 9, 2022; and the collapse of FTX on November 8, 2022.}
    \label{fig:tvr_stack_Total}
\end{figure}

==> Exhibits/wrapped_token_lst.tex <==
\begin{table}[tb] 
  \caption{Wrapped tokens in Ethereum}
    \begin{center}
    \begin{multicols*}{2} % 开始两栏环境
          \input{Tables/wrapped_tokens_list}
    \end{multicols*}
    \end{center}
    \label{tab:wrapped_tokens_list}
\end{table}

==> Headers/authors.tex <==
\author{Yichen Luo}
\affiliation{%
  \institution{UCL, Centre for Blockchain Technologies}
  \city{London}
  \country{UK}}
\email{yichen.luo.22@ucl.ac.uk}

\author{Yebo Feng}
\affiliation{%
  \institution{Nanyang Technological University}
  \country{Singapore}}
\email{yebo.feng@ntu.edu.sg}

\author{Jiahua Xu}
\affiliation{%
  \institution{UCL, Centre for Blockchain Technologies\\
  DLT Science Foundation}
  \city{London}
  \country{UK}}
\email{jiahua.xu@ucl.ac.uk}

\author{Paolo Tasca}
\affiliation{%
  \institution{UCL, Centre for Blockchain Technologies\\
  DLT Science Foundation}
  \city{London}
  \country{UK}}
\email{p.tasca@ucl.ac.uk}

==> Headers/poster-packages.tex <==
\usepackage{acro}
\usepackage{subcaption}
\usepackage{tikz}

\usepackage[english]{babel}
\setbeamersize{text margin left=2cm,text margin right=2cm}

\newlength\blockcolsep%
\setlength\blockcolsep{2ex}
\newlength\postercolumnsep%
\setlength\postercolumnsep{2cm}

\newlength\postercolumnwidth%
\setlength\postercolumnwidth{0.3333\textwidth-0.66666\postercolumnsep}

\newlength\totalwidth%
\setlength\totalwidth{\textwidth+3ex}

==> Headers/slide-packages.tex <==
\usepackage{graphicx} % Allows including images
\usepackage{booktabs} % Allows the use of \toprule, \midrule and \bottomrule in tables
\usepackage{media9}
\usepackage{hyperref}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{multicol}
\hypersetup{colorlinks=true,
	linkcolor=cyan,
	citecolor=blue,
	urlcolor=green}
 
\usepackage[ruled]{algorithm2e}
\usepackage{makecell}
\usepackage{acro}
\usepackage{tabularx}
\usepackage{tikz}
\usepackage{hhline}
\usepackage{xcolor,colortbl}
\usepackage{wasysym}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{bm}
\usepackage{csquotes}

\PassOptionsToPackage{table,xcdraw}{xcolor}

\newcommand\encircle[1]{%
  \tikz[baseline=(X.base)] 
    \node (X) [draw, shape=circle, inner sep=0.1, fill=black, text=white, font=\scriptsize] {\strut #1};%
}


==> Headers/temp-packages.tex <==
\usepackage{acm-ec-24}

==> Slides/conclusion.tex <==
\begin{frame}{Key takeaways}
\begin{itemize}
    \item Due to its sensitivity to double-counting, \acf{tvl} is a flawed, manipulatable metric for \ac{defi} value (and performance).
    \item \ac{defi} value can be more reliably measured through \acf{tvr} using accounting principles.
    \item \ac{tvr} is more stable during market downturn than \ac{tvl}.
    \item \ac{defi} multiplier $\frac{TVR}{TVL}$ can be constructed analogous to \ac{trafi} multiplier $\frac{M0}{M2}$.
    \item \ac{defi} multiplier can be a proxy for protocol complexity.
\end{itemize}
\end{frame}

==> Slides/empirical_measurement_results.tex <==
\begin{frame}{Empirical Measurement Results: TVL and TVR}
    \begin{itemize}
        \item Our measurement finds substantial
    double counting in DeFi. 
        \item DeFiLlama's adjusted TVL cannot reflect the true value of DeFi.
    \end{itemize}
    \begin{figure}
        \centering
        \includegraphics[width=0.8\linewidth]{Figures/tvl_Total.pdf}
        \caption{\footnotesize Unadjusted \ac{tvl} (red line), DeFiLlama-adjusted \ac{tvl} (blue line), and \ac{tvr} (black line).}
        \label{fig:tvl_Total}
    \end{figure}
\end{frame}

% \begin{frame}{Empirical Measurement Results: Protocol-Level TVR}
%     \begin{itemize}
%         \item \small We can find intra-protocol double counting in both Lido and Aave V2.
%     \end{itemize}
%     \begin{figure}
%         \centering
%         \begin{subfigure}{0.5\linewidth}
%           \centering
%           \includegraphics[width=\linewidth]{Figures/ind_lido.pdf}
%           \caption{Lido.}
%           \label{subfig:ind_lido}
%         \end{subfigure}%
%         \begin{subfigure}{0.5\linewidth}
%           \centering
%           \includegraphics[width=\linewidth]{Figures/ind_aave.pdf}
%           \caption{Aave V2.}
%           \label{subfig:ind_aave}
%         \end{subfigure}
%         \caption{\tiny Total receivables, total payables, and \ac{tvr} of Lido and Aave V2 in the Ethereum. The green area represents the value of total receivables, the red area denotes the value of total payables, and the blue line illustrates the protocol \ac{tvl}.}
%         \label{fig:ind_tvl}
%     \end{figure}
% \end{frame}

\begin{frame}{Empirical Measurement Results: Decomposition of TVL and TVR}
    \begin{itemize}
        \item The dominance of the top four
protocols increases following the LUNA and FTX collapses, while the double-counting proportion decreases after these events. 
    \end{itemize}
    \begin{figure}[tb]
    \centering
    \begin{subfigure}{0.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/tvl_decompose_sankey_max_tvl.pdf}
        \caption{TVL reaches the maximum value during the sample period.}
        \label{subfig:tvl_decompose_sankey_max_tvl}
    \end{subfigure}%
    \begin{subfigure}{0.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/tvl_decompose_sankey_luna_collapse.pdf}
        \caption{The end of the date of LUNA collapse.}
        \label{subfig:tvl_decompose_sankey_luna_collapse}
    \end{subfigure}%
    \begin{subfigure}{0.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/tvl_decompose_sankey_ftx_collapse.pdf}
        \caption{The end of the date of FTX collapse.}
        \label{subfig:tvl_decompose_sankey_ftx_collapse}
    \end{subfigure}
    \caption{\footnotesize Decomposition of TVL of the entire DeFi system. We identify four protocols with the highest \ac{tvl} and group the remaining protocols under the category of "Others". The band width represents the dollar value of tokens. The blue band represents the \ac{tvl} value, while the orange band represents the \ac{tvr} value.}
    \label{fig:tvl_decompose_sankey}
    \end{figure}
\end{frame}

\begin{frame}{Empirical Measurement Results: Network Analysis}
    \begin{itemize}
        \item \small We observe that both TVL and TVL-to-TVR ratio of protocols excluding Lido decreases from the point when TVL reaches the maximum value to the collapse of LUNA and FTX.
    \end{itemize}
    \begin{figure}[tb]
\centering
    \begin{subfigure}{0.33\linewidth}
          \centering
          \includegraphics[width=\linewidth]{Figures/network_max_tvl.pdf}
          \caption{\ac{tvl} reaches the maximum value during the sample period.}
          \label{subfig:network_max_tvl}
        \end{subfigure}%
        \begin{subfigure}{0.33\linewidth}
          \centering
          \includegraphics[width=\linewidth]{Figures/network_luna_collapse.pdf}
          \caption{The end of the date of LUNA collapse.}
          \label{subfig:network_luna_collapse}
        \end{subfigure}%
        \begin{subfigure}{0.33\linewidth}
          \centering
          \includegraphics[width=\linewidth]{Figures/network_ftx_collapse.pdf}
          \caption{The end of the date of FTX collapse.}
          \label{subfig:network_ftx_collapse}
        \end{subfigure}
    
    \caption{\scriptsize Token wrapping network of six representative protocols. Node size corresponds to the \ac{tvl}, edge width represents the dollar amount of tokens generated from the source protocol and staked in the target protocol, and node color reflects the ratio between \ac{tvl} and \ac{tvr}. A darker color indicates a higher level of double counting within the \ac{defi} protocol.}
    \label{fig:protocol_network}    
    \end{figure}
\end{frame}

\begin{frame}{Empirical Measurement Results: Sensitivity Tests}
    \begin{itemize}
        \item \small We further show that TVR is a more stable metric than TVL, especially during market downturns. A 25\% decline in the price of Ether (ETH) leads to a \$1 billion greater non-linear decrease in TVL compared to TVR.
    \end{itemize}
    \begin{figure}
        \centering
        \tiny
        \begin{subfigure}{0.3\linewidth}
            \centering
            \tikz\node[inner sep=0pt,
                   label=west:\rotatebox{90}{\tiny\textbf{Maximum \ac{tvl}, 2021-12-26}}]{\includegraphics[width=0.8\linewidth]{Figures/sensitivity_max_tvl_aave_c.pdf}};
            \label{subfig:sensitivity_max_tvl_aave_c}
        \end{subfigure}%
        \begin{subfigure}{0.3\linewidth}
            \centering
            \includegraphics[width=0.8\linewidth]{Figures/sensitivity_max_tvl_mkr_c.pdf}
            \label{subfig:sensitivity_max_tvl_mkr_c}
        \end{subfigure}%
        \begin{subfigure}{0.3\linewidth}
            \centering
            \includegraphics[width=0.8\linewidth]{Figures/sensitivity_max_tvl_gas.pdf}
            \label{subfig:sensitivity_max_tvl_gas}
        \end{subfigure}\\
        
        \begin{subfigure}{0.3\linewidth}
            \centering
            \tikz\node[inner sep=0pt,
                   label=west:\rotatebox{90}{\tiny\textbf{Luna collapse, 2022-05-09}}]
            {\includegraphics[width=0.8\linewidth]{Figures/sensitivity_luna_collapse_aave_c.pdf}};
            \label{subfig:sensitivity_luna_collapse_aave_c}
        \end{subfigure}%
        \begin{subfigure}{0.3\linewidth}
            \centering
            \includegraphics[width=0.8\linewidth]{Figures/sensitivity_luna_collapse_mkr_c.pdf}
            \label{subfig:sensitivity_luna_collapse_mkr_c}
        \end{subfigure}%
        \begin{subfigure}{0.3\linewidth}
            \centering
            \includegraphics[width=0.8\linewidth]{Figures/sensitivity_luna_collapse_gas.pdf}
            \label{subfig:sensitivity_luna_collapse_gas}
        \end{subfigure}\\
    \end{figure}
\end{frame}

\begin{frame}{Empirical Measurement Results: Sensitivity Tests}
    \begin{figure}
        \centering
        
        \begin{subfigure}{0.3\linewidth}
            \centering
            \tikz\node[inner sep=0pt,
                   label=west:\rotatebox{90}{\tiny\textbf{FTX collapse, 2022-05-09}},
                   label=below:\tiny\textbf{Close factor, Aave V2}]
            {\includegraphics[width=0.8\linewidth]{Figures/sensitivity_ftx_collapse_aave_c.pdf}};
            \label{subfig:sensitivity_ftx_collapse_aave_c}
        \end{subfigure}%
        \begin{subfigure}{0.3\linewidth}
            \centering
            \tikz\node[inner sep=0pt,
                   label=below:\tiny\textbf{Close factor, MakerDAO}]
            {\includegraphics[width=0.8\linewidth]{Figures/sensitivity_ftx_collapse_mkr_c.pdf}};
            \label{subfig:sensitivity_ftx_collapse_mkr_c}
        \end{subfigure}%
        \begin{subfigure}{0.3\linewidth}
            \centering
            \tikz\node[inner sep=0pt,
                   label=below:\tiny\textbf{Gas fee}]
            {\includegraphics[width=0.8\linewidth]{Figures/sensitivity_ftx_collapse_gas.pdf}};
            \label{subfig:sensitivity_ftx_collapse_gas}
        \end{subfigure}%
        
        \caption{\footnotesize Change in \ac{tvl} $\Delta_{TVL}$ and \ac{tvr} $\Delta_{TVR}$ as a function of ETH price decline in percentage $d$ on three representative point with different parameter values. Subfigures within a row represent sensitivity tests conducted under the same snapshot, whereas subfigures within a column display sensitivity tests implemented under three different sets of values for a given parameter.}
        \label{fig:sensitivity_test}
    \end{figure}
\end{frame}

\begin{frame}{Mapping between TradFi and DeFi}
    \begin{itemize}
        \item Similar to the money multiplier in \ac{trafi}, we construct the \ac{defi} money multiplier by dividing \ac{tvl} by \ac{tvr} to quantify the level of double counting.
    \end{itemize}
        \begin{table}
        \centering
        \tiny
        \renewcommand{\arraystretch}{0.5}
        \caption{\footnotesize Spearman's rank correlation coefficients between macroeconomic indicators, cryptocurrency market indicators, and \ac{defi} money multiplier computed from \ac{tvl} and \ac{tvr}. *, **, and *** denote the 1\%, 5\%, and 10\% significance levels, respectively.}
        \input{Tables/corr}
        \end{table}
        \tiny Notes: $M^{Tradfi}_t$ denotes the TradFi money multiplier, while $M^{DeFi}_t$ denotes the DeFi money multiplier. $CPI_t$ represents the Consumer Price Index. $VIX_t$ represents CBOE Volatility Index. $S\&P_t$ denotes S\&P Cryptocurrency Broad Digital Market Index, $Gas_t$ denotes Ethereum gas price, and $ETH_t$ denotes Ether price. 
\end{frame}

\begin{frame}{Altchain Analysis: Hedera}
    \begin{itemize}
        \item Compared to the networks in Ethereum mentioned, Hedera has a simpler token-wrapping network, thus experiencing less double counting under the TVL framework.
    \end{itemize}
    \begin{figure}[tb]
    \centering
        \begin{subfigure}{0.5\linewidth}
          \centering
          \includegraphics[width=0.9\linewidth]{Figures/hedera_network_current_date.pdf}
          \caption{Token wrapping network of Hedera on the observation date: 2024-03-01, which is the end of the sample period.}
        \end{subfigure}%
        \begin{subfigure}{0.5\linewidth}
          \centering
          \includegraphics[width=\linewidth]{Figures/tvl_hedera.pdf}
          \caption{TVL and TVR of Hedera over time.}
          \label{subfig:ind_aave}
        \end{subfigure}
    \end{figure}
\end{frame}

% \begin{frame}{Altchain Analysis: Ultron}
%     \begin{itemize}
%         \item Ultron is not subject to either intra-protocol or inter-protocol double counting problems under the TVR framework. However, DeFiLlama removes the TVL of the Ultron Staking Hub NFT protocol from Ultron’s TVL excluding double counting, as this protocol falls under the category of protocols that deposit into another protocol. DeFiLlama’s methodology is inaccurate, making the DeFillama-adjusted TVL of Ultron significantly lower than its TVR
%     \end{itemize}
%     \begin{figure}[tb]
%     \centering
%         \begin{subfigure}{0.5\linewidth}
%           \centering
%           \includegraphics[width=0.9\linewidth]{Figures/double-count_removal_ultron.png}
%           \caption{DeFiLlama removes the TVL of the Ultron Staking Hub NFT protocol from Ultron’s TVL excluding double counting.}
%         \end{subfigure}%
%         \begin{subfigure}{0.5\linewidth}
%           \centering
%           \includegraphics[width=\linewidth]{Figures/tvl_ultron.pdf}
%           \caption{TVL and TVR of Ultron over time.}
%           \label{subfig:ind_aave}
%         \end{subfigure}
%     \end{figure}
% \end{frame}

==> Slides/framework.tex <==
\begin{frame}{Research Question: Double Counting Problem in TVL}
    \scriptsize
    \begin{minipage}{0.6\linewidth}
        \begin{itemize}
            \item Origin: \textbf{DeFi composability}.
            \vspace{0.15cm}
            \item The \textbf{complexity} of user behavior in \ac{defi} ecosystem.
            \vspace{0.15cm}
            \item (Flow chart) simple summation of token value:
                \begin{itemize}
                    \item \fcolorbox{white}{gray!20}{Initial Value Deposited} $\$1,000$.
                    \item \fcolorbox{white}{green!20}{Total Value Locked (TVL)}: $\$4,713$ $\approx 5\times \$1,000$.
                \end{itemize}
            \vspace{0.15cm}
            \item This highlights a critical point that TVL can be \textbf{artificially inflated} through recursive wrapping without introducing new capital.
            \vspace{0.15cm}
            \item Most \ac{defi}-tracing websites \textbf{report only inflated TVL}, without revealing accurate underlying value of the \ac{defi}.
            \vspace{0.15cm}
        \end{itemize}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.4\linewidth}
        \begin{figure}
            \centering
            \includegraphics[width=0.8\linewidth]{Figures/complexity.pdf}
            \tiny 
        \end{figure}
    \end{minipage}
\end{frame}

\begin{frame}{Double Counting, Wrapping, and Leveraging}
    \begin{minipage}{0.55\linewidth}
        \scriptsize
        \begin{itemize}
            \item TVL double counting often results from two common operations: \textbf{wrapping} and \textbf{leveraging}.
            \item Mechanism of wrapping and leveraging, along with their corresponding TradFi analogies:
            
            \vspace{0.2cm}
            
            \item \textbf{Wrapping} (a) and Hypothecation (c)
            
                \vspace{0.2cm}
                
                (a): \fcolorbox{white}{green!20}{stETH (\$1,000)}\footnote{\tiny Counted into \fcolorbox{white}{green!20}{Total Value Locked}} $\rightarrow$ \fcolorbox{white}{green!20}{wstETH (\$1,000)} $\rightarrow$ DAI (\$571)
                
                \vspace{0.2cm}
                
                (c): Money $\rightarrow$ Note $\rightarrow$ Money
                
                \vspace{0.2cm}
                
                \item \textbf{Leveraging} in DeFi (b) and TradFi (d)  
                
                \vspace{0.2cm}
                
                (b) \fcolorbox{white}{green!20}{DAI (\$2,000)} $\rightarrow$ ETH (\$900) $\rightarrow$ \fcolorbox{white}{green!20}{DAI (\$900)}
                
                \vspace{0.2cm}
                
                (d) Real Estate $\rightarrow$ Loan $\rightarrow$ Real Estate
                
        \end{itemize}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.45\linewidth}
        \begin{figure}
            \centering
            \begin{subfigure}{.5\linewidth}
              \centering
              \includegraphics[width=0.8\linewidth]{Figures/cdp_lending.pdf}
              \caption{Wrapping.}
              \label{subfig:wrapping_defi}
            \end{subfigure}%
            \begin{subfigure}{.5\linewidth}
              \centering
              \includegraphics[width=0.8\linewidth]{Figures/leverage.pdf}
              \caption{Leveraging in DeFi.}
              \label{subfig:leverage_defi}
            \end{subfigure}
            \begin{subfigure}{.5\linewidth}
              \centering
              \includegraphics[width=0.8\linewidth]{Figures/discounting.pdf}
              \caption{Hypothecation.}
              \label{subfig:discounting_tradfi}
            \end{subfigure}%
            \begin{subfigure}{.5\linewidth}
              \centering
              \includegraphics[width=\linewidth]{Figures/financial_leverage.pdf}
              \caption{Leveraging in TradFi.}
              \label{subfig:leverage_tradfi}
            \end{subfigure}
        \end{figure}
    \end{minipage}
\end{frame}

\begin{frame}{TVL Double Counting: A Balance Sheet Approach}
    \scriptsize
    \begin{itemize}
        \item A \textbf{balance sheet} describes the financial position for each protocol. The aggregate value locked can be regarded as a significant element on the asset side. 
        
        \item For a DeFi ecosystem, we apply the \textbf{consolidated balance sheet} to illustrate the financial status on an aggregated basis. Non-duplication principle: entries regarded as assets in one company and liabilities in another can be eliminated. 
        \item \textbf{Wrapping Scenario}: \fcolorbox{white}{green!20}{stETH (\$1,000)} $\rightarrow$ \fcolorbox{white}{green!20}{wstETH (\$1,000)} $\rightarrow$ DAI (\$571) 
    \end{itemize}
        \begin{table}
            \centering
            \tiny
            % \caption{Protocol-perspective balance sheets and dynamics of TVL of the wrapping scenario. We highlight the \ac{tvl} and value locked in red.}
            \label{tab:consolidated-balance-sheet}
            \begin{minipage}{0.3\linewidth}
            \centering
            \caption{The \textbf{balance sheet} of Lido.}
            \label{subtab:balance-sheet-lido}
            \begin{tabular}{@{}p{0.55\linewidth}>{\raggedleft\arraybackslash}p{0.14\linewidth}>{\raggedleft\arraybackslash}p{0.17\linewidth}@{}}
                \toprule
                \textbf{Immediately After} & \encircle{2} & \encircle{4} \\
                \midrule
                \textit{Assets} & \$ & \$ \\
                \fcolorbox{white}{green!20}{Value Locked - stETH} & \textcolor{green}{1,000} & \textcolor{green}{1,000} \\
                &&\\
                \midrule
                \textbf{Total Assets} & 1,000 & 1,000 \\
                \bottomrule\bottomrule
                \textit{Liabilities} & \$ & \$ \\
                Payables - wstETH & 1,000 & 1,000 \\
                &&\\
                \midrule
                \textbf{Total Liabilities} & 1,000 & 1,000 \\
                \bottomrule\bottomrule
            \end{tabular}
            \end{minipage}%
            \hfill
            \begin{minipage}{0.3\linewidth}
            \centering
            \caption{The \textbf{balance sheet} of MakerDAO.}
            \label{subtab:balance-sheet-makerdao}
            \begin{tabular}{@{}p{0.55\linewidth}>{\raggedleft\arraybackslash}p{0.14\linewidth}>{\raggedleft\arraybackslash}p{0.17\linewidth}@{}}
                \toprule
                \textbf{Immediately After} & \encircle{2} & \encircle{4} \\
                \midrule
                \textit{Assets} & \$ & \$ \\
                \fcolorbox{white}{green!20}{Value Locked - wstETH} & - & \textcolor{green}{1,000} \\
                Receivables - DAI & - & 571 \\
                \midrule
                \textbf{Total Assets} & - & 1,571 \\
                \bottomrule\bottomrule
                \textit{Liabilities} & \$ & \$ \\
                Payables - wstETH & - & 1,000 \\
                New Money - DAI & - & 571 \\
                \midrule
                \textbf{Total Liabilities} & - & 1,571 \\
                \bottomrule\bottomrule
            \end{tabular}
            \end{minipage}%
            \hfill
            \begin{minipage}{0.3\linewidth}
            \centering
            \caption{\textbf{Consolidated balance sheet} of Lido and MakerDAO.}
            \label{subtab:consolidated-balance-sheet}
            \begin{tabular}{@{}p{0.45\linewidth}>{\raggedleft\arraybackslash}p{0.14\linewidth}>{\raggedleft\arraybackslash}p{0.17\linewidth}@{}}
                \toprule
                \textbf{Immediately After} & \encircle{2} & \encircle{4} \\
                \midrule
                \textit{Assets} & \$ & \$ \\
                \fcolorbox{white}{gray!20}{Value Locked} & \textcolor{gray}{1,000} & \textcolor{gray}{1,000} \\
                Receivables & - & 571 \\
                \midrule
                \textbf{Total Assets} & 1,000 & 1,571 \\
                \bottomrule\bottomrule
                \textit{Liabilities} & \$ & \$ \\
                Payables & 1,000 & 1,571 \\
                &&\\
                \midrule
                \textbf{Total Liabilities} & 1,000 & 1,571 \\
                \bottomrule\bottomrule
            \end{tabular}
            \end{minipage}
            \end{table}
\end{frame}

\begin{frame}{TVL Double Counting: A Balance Sheet Approach}
    \begin{itemize}
        \item \textbf{Leveraging Scenario}: \fcolorbox{white}{green!20}{DAI (\$2,000)} $\rightarrow$ ETH (\$900) $\rightarrow$ \fcolorbox{white}{green!20}{DAI (\$900)}
    \end{itemize}
        \begin{table}[tb]
            \centering
            \tiny
            % \caption{Protocol-perspective balance sheets and dynamics of TVL of the leveraging scenario. We highlight the \ac{tvl} in red.}
            \label{tab:consolidated-balance-sheet-2}
            \begin{minipage}{0.3\linewidth}
            \centering
            \caption{The \textbf{balance sheet} of Aave.}
            \label{subtab:balance-sheet-curve}
            \begin{tabular}{@{}p{0.55\linewidth}>{\raggedleft\arraybackslash}p{0.14\linewidth}>{\raggedleft\arraybackslash}p{0.17\linewidth}@{}}
                \toprule
                \textbf{Immediately After} & \encircle{1} & \encircle{5} \\
                \midrule
                \textit{Assets} & \$ & \$ \\
                \fcolorbox{white}{green!20}{Value Locked - DAI} & \textcolor{green}{2,000} & \textcolor{green}{2,900} \\
                Receivables - dETH & 900 & 900 \\
                \midrule
                \textbf{Total Assets} & 2,900 & 3,800 \\
                \bottomrule\bottomrule
                \textit{Liabilities} & \$ & \$ \\
                Payables - aDAI & 2,000 & 2,900 \\
                Payables - aETH & 900 & 900\\
                \midrule
                \textbf{Total Liabilities}  & 2,000 & 3,800 \\
                \bottomrule\bottomrule
            \end{tabular}   
            \end{minipage}%
            \hfill
            \begin{minipage}{0.3\linewidth}
            \centering
            \caption{The \textbf{balance sheet} of Uniswap.}
            \label{subtab:balance-sheet-yearn}
            \begin{tabular}{@{}p{0.55\linewidth}>{\raggedleft\arraybackslash}p{0.14\linewidth}>{\raggedleft\arraybackslash}p{0.17\linewidth}@{}}
                \toprule
                \textbf{Immediately After} & \encircle{1} & \encircle{5} \\
                \midrule
                \textit{Assets} & \$ & \$ \\
                \fcolorbox{white}{green!20}{Value Locked - ETH} & \textcolor{green}{1,800} & \textcolor{green}{2,700} \\
                \fcolorbox{white}{green!20}{Value Locked - DAI} & \textcolor{green}{1,800} & \textcolor{green}{900} \\
                \midrule
                \textbf{Total Assets} & 3,600 & 3,600 \\
                \bottomrule\bottomrule
                \textit{Liabilities} & \$ & \$ \\
                Payables - ETH-DAI-LP & 3,600 & 3,600 \\
                &&\\
                \midrule
                \textbf{Total Liabilities} & 3,600 & 3,600 \\
                \bottomrule\bottomrule
            \end{tabular}
            \end{minipage}%
            \hfill
            \begin{minipage}{0.3\linewidth}
            \centering
            \caption{\textbf{Consolidated balance sheet} of Aave and Uniswap.}
            \label{subtab:consolidated-balance-sheet-2}
            \begin{tabular}{@{}p{0.45\linewidth}>{\raggedleft\arraybackslash}p{0.14\linewidth}>{\raggedleft\arraybackslash}p{0.17\linewidth}@{}}
                \toprule
                \textbf{Immediately After} & \encircle{1} & \encircle{5} \\
                \midrule
                \textit{Assets} & \$ & \$ \\
                \fcolorbox{white}{gray!20}{Value Locked} & \textcolor{gray}{5,600} & \textcolor{gray}{5,600} \\
                &&\\
                \midrule
                \textbf{Total Assets} & 5,600 & 5,600 \\
                
                \bottomrule\bottomrule
                \textit{Liabilities} & \$ & \$ \\
                Payables & 5,600 & 5,600 \\
                &&\\
                \midrule
                \textbf{Total Liabilities} & 5,600 & 5,600 \\
                \bottomrule\bottomrule
            \end{tabular}
            \end{minipage}
        \end{table}
\end{frame}


% \begin{frame}{Intra-protocol Double Counting: Account-perspective Balance Sheets}
%     \scriptsize
%     \begin{itemize}
%         \item Lido: \fcolorbox{white}{green!20}{ETH (\$1,000)} $\rightarrow$ \fcolorbox{white}{green!20}{stETH (\$1,000)} $\rightarrow$ wstETH (\$571)
%         \item  Aave: \fcolorbox{white}{green!20}{DAI (\$2,000)} $\rightarrow$ \fcolorbox{white}{green!20}{ETH (\$900)} $\rightarrow$ DAI (\$900) 
%     \end{itemize}
%     \begin{table}
%     \centering
%     \tiny
%     \begin{minipage}{0.45\linewidth}
%         \centering
%         \caption{Lido user.}
%         \label{subtab:acct_bs_wrapping}
%         \begin{tabular}{@{}p{0.45\linewidth}>{\raggedleft\arraybackslash}p{0.13\linewidth}>{\raggedleft\arraybackslash}p{0.13\linewidth}@{}}
%             \toprule
%             \textbf{Immediately After} & \encircle{2} & \encircle{4} \\
%             \midrule
%             \textit{Assets} &  \$ &  \$ \\
%             Receivables - stETH  & \textcolor{green}{1,000} & \textcolor{green}{0} \\
%             Receivables - wstETH & \textcolor{green}{-} & \textcolor{green}{1,000} \\
%             & \\
%             & \\
%             \midrule
%             \textbf{Total Assets}  & 1,000 & 1,000 \\
%             \bottomrule\bottomrule
%             \textit{Liabilities} & \$ & \$ \\
%             & \\
%             \midrule
%             \textbf{Total Liabilities} & 0 & 0 \\
%             \bottomrule
%             \textit{Net Positions} & \$ & \$ \\
%             Initial Deposit Value - ETH & 1,000 & 1,000 \\
%             \midrule
%             \textbf{Total Net Positions} & 1,000 & 1,000 \\
%             \bottomrule\bottomrule
%         \end{tabular}
%     \end{minipage}%
%     \hfill
%     \begin{minipage}{0.45\linewidth}
%         \centering
%         \caption{Aave user.}
%         \label{subtab:acct_bs_leveraging}
%         \begin{tabular}{@{}p{0.45\linewidth}>{\raggedleft\arraybackslash}p{0.13\linewidth}>{\raggedleft\arraybackslash}p{0.13\linewidth}>{\raggedleft\arraybackslash}p{0.13\linewidth}@{}}
%             \toprule
%             \textbf{Immediately After} & \encircle{0} & \encircle{3} & \encircle{5} \\
%             \midrule
%             \textit{Assets} & \$ & \$ & \$ \\
%             Cash - DAI & 2,000 & 0 & 0 \\
%             Cash - ETH & - & 900 & 0 \\
%             Receivables - aDAI & \textcolor{green}{-} & \textcolor{green}{2,000} & \textcolor{green}{2,000} \\
%             Receivables - aETH & \textcolor{green}{-} & \textcolor{green}{-} & \textcolor{green}{900} \\
%             \midrule
%             \textbf{Total Assets} & 2,000 & 2,900 & 2,900 \\
%             \bottomrule\bottomrule
%             \textit{Liabilities} & \$ & \$ & \$ \\
%             Payables - dETH & \textcolor{red}{-} & \textcolor{red}{900} & \textcolor{red}{900}\\
%             \midrule
%             \textbf{Total Liabilities}  & 0 & 0 & 0 \\
%             \bottomrule
%             \textit{Net Positions} & \$ & \$ & \$ \\
%             Initial Deposit Value - DAI & 2,000 & 2,000 & 2,000 \\
%             \midrule
%             \textbf{Total Net Positions}  & 2,000 & 2,000 & 2,000 \\
%             \bottomrule\bottomrule
%         \end{tabular}
%     \end{minipage}
%     \end{table}

% \end{frame}

\begin{frame}{Existing Methodology: DeFiLlama's Adjusted TVL}
\footnotesize
\begin{itemize}
    \item DeFiLlama-adjusted TVL is calculated by first aggregating the TVL of all eligible protocols and then summing the TVL across all blockchains, where protocol eligibility is arbitrarily determined by DeFiLlama whose validity we challenge.
\end{itemize}
    \begin{figure}
      \centering
      \includegraphics[width=0.5\linewidth]{Figures/double-count-removal.png}
      \caption{\tiny DeFiLlama's \ac{tvl} dashboard after deactivating the \enquote{Include in \ac{tvl}: Double Count} toggle. When a user deactivates this toggle, protocols that deposit into another protocol will be excluded from the total \ac{tvl} calculation, and their \ac{tvl} numbers will be displayed in grey.}
\end{figure}
\end{frame}

\begin{frame}{Enhanced Measurement Framework: Total Value Redeemable (TVR)}
    \footnotesize
    \input{Definitions/tvr}
    \begin{itemize}
        \item \acs{tvl}: \input{Equations/category_tvl}
        \item \acs{tvr} for blockchains and \ac{defi} ecosystem: \input{Equations/tvr}
        % \item \acs{tvr} for protocol: ${\it TVR}_{i} = \textstyle\sum_{j \in \mathcal{A}_{i}} R_{j} -\textstyle\sum_{j \in \mathcal{A}_{i}} P_{j},$ 
        
        % where $P_{i}$ and $R_{i}$ denote the total payables and receivables in the balance sheet of account $i$.
    \end{itemize}
\end{frame}

==> Slides/intro.tex <==
\begin{frame}{Introduction: Total Value Locked (TVL) and DeFiLlama}
% \begin{itemize}
%     \item Total Value Locked (TVL) is defined as the total value of assets staked by users in a DeFi protocol or DeFi ecosystem at a specific moment.
% \end{itemize}
    \input{Definitions/tvl}
    \begin{minipage}{0.4\linewidth}
        \footnotesize
        \begin{itemize}
            \item Similar to \textbf{AUM} in TradFi, \textbf{TVL} is widely used to indicate the \textbf{size and popularity} of DeFi ecosystem.
            \vspace{0.2cm}
            \item TVL figures are reported by DeFi-tracing websites, with \textbf{DeFiLlama} being the most widely recognized one.
        \end{itemize}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.6\linewidth}
        \begin{figure}
            \centering
            \includegraphics[width=\linewidth]{Figures/defillama_panel.png}
            \scriptsize 
            \caption{Screenshot of DeFiLlama TVL Dashboard.}
            \label{fig:tvl_Total}
        \end{figure}
    \end{minipage}
    
\end{frame}


==> Slides/outline.tex <==
\begin{frame}{Outline}
    \tableofcontents    
\end{frame}

==> Slides/outtro.tex <==
\begin{frame}{Thank you}

Yichen Luo

yichen.luo.22@ucl.ac.uk

\end{frame}

==> Slides/title.tex <==
\begin{frame}
    \titlepage
\end{frame}

==> Tables/dyn_curve_yearn.tex <==
\begin{tabular}{@{}p{0.57\linewidth}p{0.10\linewidth}p{0.13\linewidth}@{}}
\toprule
& \textbf{$\mathcal{S}^{(1)}_{\textnormal{L}}$} & \textbf{$\mathcal{S}^{(3)}_{\textnormal{L}}$}\\
\midrule
& \$ & \$ \\
&&\\
&&\\
&&\\
&&\\
&&\\
\midrule
\textbf{Total Value Locked} & \textcolor{red}{5,600} & \textcolor{red}{6,500}\\
\bottomrule\bottomrule
\end{tabular}

==> Tables/dyn_makerdao_aave.tex <==
\begin{tabular}{@{}p{0.50\linewidth}p{0.14\linewidth}p{0.17\linewidth}@{}}
\toprule
& \textbf{$\mathcal{S}^{(1)}_{\textnormal{W}}$} & \textbf{$\mathcal{S}^{(2)}_{\textnormal{W}}$} \\
\midrule
& \$ & \$ \\
&&\\
&&\\
&&\\
&&\\
&&\\
&&\\
\midrule
\textbf{Total Value Locked} & \textcolor{red}{1,000} & \textcolor{red}{2,000} \\
\bottomrule\bottomrule
\end{tabular}
